Some minimal bimolecular mass-action systems with limit cycles

We discuss three examples of bimolecular mass-action systems with three species, due to Feinberg, Berner, Heinrich, and Wilhelm. Each system has a unique positive equilibrium which is unstable for certain rate constants and then exhibits stable limit cycles, but no chaotic behaviour. For some rate constants in the Feinberg--Berner system, a stable equilibrium, an unstabe limit cycle, and a stable limit cycle coexist. All three networks are minimal in some sense. By way of homogenising the above three examples, we construct bimolecular mass-conserving mass-action systems with four species that admit a stable limit cycle. The homogenised Feinberg--Berner system and the homogenised Wilhelm--Heinrich system admit the coexistence of a stable equilibrium, an unstable limit cycle, and a stable limit cycle.

==> sections/6_L1.tex <==
\section{Stability of an equilibrium} \label{sec:app}

In this section we collect a few known results related to the stability of an equilibrium of a three-dimensional differential equation, cf.\ \cite[Section 5.4]{kuznetsov:2004}. In particular, we present formula \eqref{eq:L1n3_canonical} below, which is used in the main text a couple of times.

We start by recalling the Routh--Hurwitz criterion for a cubic polynomial $\lambda^3 + a_2 \lambda^2 + a_1 \lambda + a_0$:
\begin{enumerate}[(i)]
    \item all three roots have negative real part if and only if $a_0>0$, $a_2>0$, $a_2a_1>a_0$,
    \item the three roots are $\omega i$, $-\omega i$, $\varrho$ with $\varrho<0$ and $\omega>0$ if and only if $a_0>0$, $a_2>0$, $a_2a_1=a_0$.
\end{enumerate}

We now sketch how to bring a matrix $J\in\mathbb{R}^{3 \times 3}$ with eigenvalues $\omega i$, $-\omega i$, $\varrho$ (where $\varrho$ and $\omega$ are nonzero real numbers) to canonical form. Since $\omega i$ is an eigenvalue of $J$ (and of $J^\top$), the real number $-\omega^2$ is an eigenvalue of $J^2$ (and of $(J^\top)^2$). Let $v_1, v_2, v_3 \in \mathbb{R}^3\setminus \{0\}$ be such that 
\begin{align*}
(J^\top)^2v_1 &= -\omega^2 v_1,\\
J^\top v_1 &= -\omega v_2,\\
J^\top v_3 &= \varrho v_3.
\end{align*}
Let the $i$th row of the matrix $T \in \mathbb{R}^{3 \times 3}$ be $v_i^\top$. Then it is straightforward to check that
\begin{align*}
TJT^{-1}=\begin{bmatrix}
0 & -\omega & 0 \\ \omega & 0 & 0 \\ 0 & 0 & \varrho
\end{bmatrix}.
\end{align*}

With $\omega,\varrho\in\mathbb{R}\setminus\{0\}$, for the differential equation
\begin{align}\label{eq:app_canonical_ode}
\begin{split}
\dot{x} &= -\omega y + \frac12 \left[f_{200}x^2 + 2 f_{110}xy + f_{020}y^2 + 2f_{101}xz + 2f_{011}yz+\cdots\right] +\\
&\quad + \frac16 \left[f_{300}x^3+3f_{120}xy^2+\cdots\right]+\text{h.o.t.},  \\
\dot{y} &= \omega x + \frac12 \left[g_{200}x^2 + 2 g_{110}xy + g_{020}y^2 + 2g_{101}xz + 2g_{011}yz +\cdots\right] +\\
& \quad + \frac16 \left[3g_{210}x^2y + g_{030}y^3+\cdots\right]+\text{h.o.t.}, \\
\dot{z} &= \varrho z + \frac12[h_{200}x^2 + 2 h_{110}xy + h_{020}y^2+\cdots]+\text{h.o.t.},
\end{split}
\end{align}
the origin is an equilibrium with eigenvalues $\omega i$, $-\omega i$, $\varrho$. The first focal value, $L_1$, there is given by
\begin{align}\label{eq:L1n3_canonical}
\begin{split}
&L_1 = f_{300} + f_{120} + g_{030} + g_{210} +\\ &\quad+\frac1{\omega}\left[f_{110}(f_{200}+f_{020})-g_{110}(g_{200}+g_{020})+f_{020}g_{020}-f_{200}g_{200}\right]-\\
&\quad-\frac{h_{200}}{\varrho\left(\varrho^2+4\omega^2\right)}\left[(3\varrho^2+8\omega^2)f_{101} - 2\varrho\omega f_{011} - 2\varrho\omega g_{101} + (\varrho^2+8\omega^2)g_{011}\right]-\\
&\quad-\frac{2h_{110}}{\varrho^2+4\omega^2}\left[2\omega f_{101} + \varrho f_{011} + \varrho g_{101}-2\omega g_{011}\right]-\\
&\quad-\frac{h_{020}}{\varrho\left(\varrho^2+4\omega^2\right)}\left[(\varrho^2+8\omega^2)f_{101} + 2\varrho\omega f_{011} + 2\varrho\omega g_{101} + (3\varrho^2+8\omega^2)g_{011}\right].
\end{split}
\end{align}
We now briefly explain how to derive this formula. Let us consider the quadratic approximation of the center manifold:
\begin{align}\label{eq:app_center_manifold}
z = \frac{1}{2}[c_{20} x^2 + 2c_{11} xy + c_{02} y^2] + \text{h.o.t.}
\end{align}
To find $c_{20}$, $c_{11}$, $c_{02}$, differentiate both sides of \eqref{eq:app_center_manifold} w.r.t.\ time and thus find that
\begin{align}\label{eq:app_zdot1}
\begin{split}
\dot{z} &= c_{20} x \dot{x} + c_{11}(\dot{x} y + x \dot{y}) + c_{02} y \dot{y} + \text{h.o.t.}=\\
&=-\omega c_{20} xy + \omega c_{11}(-y^2+x^2) + \omega c_{02} xy + \text{h.o.t.}
\end{split}
\end{align}
On the other hand, from \eqref{eq:app_canonical_ode}, we find that on the center manifold
\begin{align}\label{eq:app_zdot2}
\dot{z} = \frac12[(\varrho c_{20} + h_{200})x^2 + 2(\varrho c_{11} + h_{110})xy + (\varrho c_{02} + h_{020})y^2]+ \text{h.o.t.}
\end{align}
Equating the coefficients of $x^2$, $xy$, $y^2$ in \eqref{eq:app_zdot1} and \eqref{eq:app_zdot2} gives a system of three linear equations for the three unknowns $c_{20}$, $c_{11}$, $c_{02}$. After solving that, plug in $z = \frac{1}{2}[c_{20} x^2 + 2c_{11} xy + c_{02} y^2]$ to $\dot{x}$ and $\dot{y}$ in \eqref{eq:app_canonical_ode}. This gives the dynamics on the two-dimensional center manifold and one can then apply the planar first focal value formula to obtain \eqref{eq:L1n3_canonical}.
